Mori-Zwanzig mode decomposition: Comparison with time-delay embeddings

We introduce the Mori-Zwanzig Mode Decomposition (MZMD), a novel data-driven technique for efficient modal analysis of and reduced-order modeling of large-scale spatio-temporal dynamical systems. MZMD represents an extension of Dynamic Mode Decomposition (DMD) by providing an approximate closure term with MZ memory kernels accounting for how the unresolved modes of DMD interact with the resolved modes, thus addressing limitations when the state-space observables do not form a Koopman-invariant subspace. Leveraging the Mori-Zwanzig (MZ) formalism, MZMD identifies the modes and spectrum of the discrete-time Generalized Langevin Equation (GLE); an integro-differential equation that governs the dynamics of selected observables and their memory-dependent coupling with the unresolved degrees of freedom. This feature fundamentally distinguishes MZMD from time-delay embedding methods, such as Higher-Order DMD (HODMD). In this work, we derive and analyze MZMD and compare it with DMD and HODMD, using two exemplary Direct Numerical Simulation (DNS) datasets: a 2D flow over a cylinder (as validation) and laminar-turbulent boundary-layer transition over a flared cone at Mach 6. We demonstrate that MZMD, via the addition of MZ memory terms, improves the resolution of spatio-temporal structures within the transitional/turbulent regime by the introduction of transient and periodic modes (not captured by DMD), which contain features that arise due to nonlinear mechanisms, such as the generation of the so-called hot streaks on the surface of the flared cone. Our results demonstrate that MZMD serves as an efficient generalization of DMD (reducing to DMD in the absence of memory), improves stability, and exhibits greater robustness and resistance to overfitting compared to HODMD.

==> sections/cylinder_results.tex <==
\section{Numerical results: 2D flow over cylinder}
\label{sec:2d_cylinder}


In this section, we provide a numerical comparison between DMD, HODMD, and MZMD for a two-dimensional flow over a cylinder. In this work, this flow serves as a simple test-bed for validation, performing analysis and comparisons. The flow past a two-dimensional cylinder at low Reynolds numbers results in periodic structures in the wake. The wake forms a pattern of alternating vortices, commonly referred to as a von Kármán vortex street. This vortex street over a cylinder has been extensively studied \citep{Tritton_1959, Dennis_Chang_1970, LINNICK2005157, colonius2008}. In this work, we use both $Re=200$ and $Re=600$ to investigate the effects of adding time-delay embeddings vs MZ memory, where both forms of memory are also combined. 

In figure \ref{fig:dns_cylinder} we show a snapshot of the vorticity, which was obtained by the use of the immersed boundary projection method developed by \citet{colonius2008}. We consider the statistically stationary flow obtained after the initial transient that evolves from the unstable equilibrium point to the equilibrium point representing the von Kármán vortex street. For the numerical simulation we use $dt=0.01$ (s), which is sampled every $10^{th}$ time step. The wake shedding frequency is approximately $f_s \approx 0.23$ (Hz), associated with the dominant coherent structure of the flow. In our study, we also consider the first and second higher harmonics (i.e. $2f_s$, and $3f_s$ respectively) that are present in this flow.  This flow exhibits low rank structure as seen in the total variation contained in the first dominant POD modes shown in figure \ref{fig:dns_cylinder}. We see that using more than 15 POD modes captures over $99\%$ of the variation in the vorticity field.


We first compare DMD, HODMD, and MZMD for their diagnostic capabilities, extracting dominant modes and spectrum. We show that in the case where DMD is truncated (with $r=5$), so that it does not capture the first higher harmonic, adding MZ memory (or time-delay embedding) can recover this missing dominant mode. This is associated with a dominant periodic mode occurring at the first higher harmonic (i.e. $2f_s$) which is capture by including memory. (Should we include power spectrum?). 

Next we demonstrate the differences in the algorithms of HODMD and MZMD.  HODMD and MZMD can result in different block companion matrices. For example, the second SVD that occurs in HODMD (recall from section \ref{sec:hodmd}) can result in truncation errors that lead to breaking the original formulation of HODMD, with the non-diagonal terms breaking the "higher-order" Koopman assumption of HODMD. We also see that the memory terms that are obtained with HODMD can grow, which is nonphysical, as physical processes exhibit decaying cross corelation in time. Whereas, MZMD does have the decay of memory as expected from this system. Furthermore, MZMD is much less expensive, nearly an order of magnitude less expensive than HODMD. Additionally, the learned companion matrices of MZMD converge faster with increasing number of samples, compared with HODMD. 

Next we compare the prediction accuracies of both future state prediction and out of sample generalization erro given a new initial condition. We see that MZMD can achieve better results for some cases, but typically both converge to the same result for this flow. Next, we see where memory can play an important role, namely, when there is a truncated DMD (r small enough) memory can compensate for this to obtain the appropriate spectral content. DMD can miss the higher harmonic modes with truncated r, and for this same truncation in r, adding MZ memory (or time-delay embedding with HODMD) can capture this missing mode. all methods do capture well the shedding frequency and first two higher harmonics when r is large enough (or memory is large enough). Furthermore, the modes shapes are slightly different between these three methods, especially near the immediate wake of the cylinder.  

\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.55\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dns_snapshot_2.png}
\end{subfigure}
\begin{subfigure}[]{0.44\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/pod_mode_energy_ts3_r20_k1.png}
\end{subfigure}
\caption{Snapshot of 2D flow over cylinder (left). Energy contained in POD modes (right).} 
\label{fig:dns_cylinder}
\end{figure}

First we investigate the ability of the HODMD and MZMD methods to preserve the block companion structure, which is necessary to satisfy the higher order Koopman assumption \eqref{eq:hodmd_assumption}. In figure \ref{fig:R_tilde_cylinder}, we see that this companion structure can be broken in HODMD, for example, if the second SVD is truncated, which is guaranteed to occur if not enough time snapshots $T$ are provided, namely if $T \leq dr_1$. However, by construction, we see MZMD retains this structure. What also becomes apparent in this figure, is that MZMD memory decays, whereas HODMD memory does not. This is indicative of a memory model that is less physically grounded, since physical systems exhibit decaying two-time correlation \textcolor{blue}{Cite and explain more of previous sentence. ??In this case, we see that HODMD is merely memorizing past history?? }. In figure \ref{fig:R_tilde_cylinder} we see that the relative contribution of the memory terms in MZMD is decaying, and nontrivial up to $k \approx 15$, which can be used as a memory length selection criterion.


\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.3\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/R_tilde_companion_nd6_r15_tend133_ts3.png}
\caption{Full $SVD_2$}
\end{subfigure}
\centering
\begin{subfigure}[]{0.3\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/R_tilde_companion_nd6_r15_tend80_ts5.png}
\caption{Truncated $SVD_2$}
\end{subfigure}
\begin{subfigure}[]{0.3\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/Cg_companion_k6_r15_tend1200.png}
\caption{MZMD companion $\bm C^{(g)}$}
\end{subfigure}

\centering
\begin{subfigure}[]{0.35\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/memory_decay_comparison_cylinder.png}
\caption{Memory vs time-delays}
\end{subfigure}
\caption{Checking the block companion structure of HODMD and MZMD. (b) When the second SVD in HODMD is truncated the higher order Koopman assumption is invalid as seen in the non-zeros terms outside of the block companion. (d) Compares HODMD with MZMD for flow over 2D cylinder over 20 samples representing different training data sets demonstrating memory decay where blue $\star$ is MZMD, and black $\square$ is HODMD.} 
\label{fig:R_tilde_cylinder}
\end{figure}



Next, we investigate the ability of DMD, HODMD, and MZMD to make future state predictions with varying r. Figure \ref{fig:cyl_gen_errx0} shows the future state prediction over 40 samples drawn independently from a long statistically stationary flow with $Re=600$. Each prediction is made with an $\bm z_0$ that is time shifted from the final snapshot in time from the training set. We see in this figure that for each fixed r, the relative $L_2$ future state prediction errors decreases over DMD (no memory) by adding memory for both MZMD and HODMD. Although HODMD converges faster than MZMD, adding MZ memory can eventually improve upon HODMD. Additionally in this figure, we see that the inclusion of a single time delay within MZMD demonstrates that adding MZ memory on top of time-delay embedding can improve the results. With MZMD, we see that there is a significant improvement by adding MZ memory. Additionally, as reported in figure \ref{fig:costs_convergence}, this is achieved at nearly the same computational cost as DMD. Furthermore, MZMD is nearly an order of magnitude less computationally expensive than HODMD, due to HODMD performing an additional SVD. Both costs are dominated by the initial SVD which is removed from this analysis in order to show the direct comparison of the core algorithms.



%prediction errors from new independent sample of initial conditions.
\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dominant_modes_test_error_amx0_max_gen_UQ_over_k_vs_d_lines_dts2_r3_t1_re600.png}
\caption{$r=3$}
\label{fig:cyl_gen_errx0_r10}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dominant_modes_test_error_amx0_max_gen_UQ_over_k_vs_d_lines_dts2_r5_t1_re600.png}
\caption{$r=5$}
\label{fig:cyl_gen_errx0_r20}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dominant_modes_test_error_amx0_max_gen_UQ_over_k_vs_d_lines_dts2_r7_t1_re600.png}
\caption{$r=7$}
\label{fig:cyl_gen_errx0_r30}
\end{subfigure}

\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dominant_modes_test_error_amx0_mse_gen_UQ_over_k_vs_d_lines_dts2_r3_t1_re600.png}
\caption{$r=3$}
\label{fig:cyl_gen_errx0_r10}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dominant_modes_test_error_amx0_mse_gen_UQ_over_k_vs_d_lines_dts2_r5_t1_re600.png}
\caption{$r=5$}
\label{fig:cyl_gen_errx0_r20}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dominant_modes_test_error_amx0_mse_gen_UQ_over_k_vs_d_lines_dts2_r7_t1_re600.png}
\caption{$r=7$}
\label{fig:cyl_gen_errx0_r30}
\end{subfigure}

\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/noise_dominant_modes_test_error_amx0_max_gen_UQ_over_k_vs_d_lines_dts2_r3_t1_re600.png}
\caption{$r=3$}
\label{fig:cyl_gen_errx0_r10}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/noise_dominant_modes_test_error_amx0_max_gen_UQ_over_k_vs_d_lines_dts2_r5_t1_re600.png}
\caption{$r=5$}
\label{fig:cyl_gen_errx0_r20}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/noise_dominant_modes_test_error_amx0_max_gen_UQ_over_k_vs_d_lines_dts2_r7_t1_re600.png}
\caption{$r=7$}
\label{fig:cyl_gen_errx0_r30}
\end{subfigure}

\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/noise_dominant_modes_test_error_amx0_mse_gen_UQ_over_k_vs_d_lines_dts2_r3_t1_re600.png}
\caption{$r=3$}
\label{fig:cyl_gen_errx0_r10}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/noise_dominant_modes_test_error_amx0_mse_gen_UQ_over_k_vs_d_lines_dts2_r5_t1_re600.png}
\caption{$r=5$}
\label{fig:cyl_gen_errx0_r20}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/noise_dominant_modes_test_error_amx0_mse_gen_UQ_over_k_vs_d_lines_dts2_r7_t1_re600.png}
\caption{$r=7$}
\label{fig:cyl_gen_errx0_r30}
\end{subfigure}

\caption{Long time (6 periods) out of sample future state predictions comparing relative generalization errors over 40 samples, using the six dominant modes (those shown in spectral analysis). Initial condition is shifted from fixed training set so that $\bm x_0$ is independent from training set. Bottom two rows includes noise ($0.15*\max{\bm G_0}N(0,1)$ in training set, making predictions without noise. } 
\label{fig:cyl_gen_errx0}
\end{figure}

Now, we compare the modes and spectrum of HODMD and MZMD. We see in figure \ref{fig:mzmd_hodmd_evals} that the time evolution of the modes are very different. With MZMD containing more transient modes that HODMD. We see that both MZMD and HODMD increase the spectral complexity over DMD for the same $r$. In figure \ref{fig:mode_comparions} we compare the modes of each method. \textcolor{blue}{Check normalization and amplitude sorting of this plot}. In this figure we report the dominant modes, as arranged in descending order from their largest to smallest amplitudes.




\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/dmd_spectrum_r5_k1.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/hodmd_spectrum_r5_k1_re600.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_spectrum_r5_k6.png}
\end{subfigure}
\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_spectrum_vs_ampr5_k1_tend1200_re600.png}
\end{subfigure}
\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/hodmd_spectrum_vs_ampr5_d6_k1_tend600_re600.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_spectrum_vs_ampr5_k6_tend1200_re600.png}
\end{subfigure}
\caption{From left to right, power spectrum of DMD, HODMD and MZMD, fixing $r=5$, with 6 memory terms. Each captures the dominant shedding frequency, however, only HODMD and MZMD can capture the both higher order harmonics.} 
\label{fig:mzmd_hodmd_evals}
\end{figure}



\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_dominatn_modes1_nk1_r5.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/hodmd_dominatn_modes1_nk1_r5_d.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_dominatn_modes1_nk6_r5_d1.png}
\end{subfigure}

\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_dominatn_modes2_nk1_r5.png}
% \caption{DMD eigenvalues}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/hodmd_dominatn_modes2_nk1_r5_d.png}
% \caption{HODMD eigenvalues}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_dominatn_modes2_nk6_r5_d1.png}
% \caption{MZMD eigenvalues}
\end{subfigure}

\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_dominatn_modes3_nk1_r5.png}
% \caption{DMD eigenvalues}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/hodmd_dominatn_modes3_nk1_r5_d.png}
% \caption{HODMD eigenvalues}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/mzmd_dominatn_modes3_nk6_r5_d1.png}
% \caption{MZMD eigenvalues}
\end{subfigure}
\caption{Comparing modes from DMD, HODMD, MZMD, with $r = 5$. Contour levels are normalized between $(-1, 1)$. DMD modes (left column), HODMD (middle column), MZMD (right column). Dominant to higher harmonics from top to bottom.} 
\label{fig:mode_comparions}
\end{figure}


\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.4\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/avg_r_comp_costs_in_g_space.png}
\caption{Computational Costs}
\label{fig:costs}
\end{subfigure}
\begin{subfigure}[]{0.4\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/convergence2_of_companions_r30_k5.png}
\caption{Convergence of operators}
\label{fig:conv}
\end{subfigure}
\caption{(\subref{fig:costs}) The computational costs between MZMD (blue $\star$), MZMD with one time delay embedding (green $\circ$), and HODMD (black $\square$) over 30 independent samples of the 2D flow over a cylinder. \subref{fig:conv} Shows MZMD requires less training data for a similar level of convergence of the respective block companion matrix. These experiments were run on an Apple M1 Max Chip.} 
\label{fig:costs_convergence}
\end{figure}


\begin{figure}[!htb]
\centering
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/convergence_of_modes_r5_k8.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/convergence_of_modes_r10_k8.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/convergence_of_modes_r20_k8.png}
\end{subfigure}
\centering
\begin{subfigure}[]{0.33\textwidth}
\includegraphics[width=1\textwidth]{figures/convergence_of_modes_noise_r5_k8.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/convergence_of_modes_noise_r10_k8.png}
\end{subfigure}
\begin{subfigure}[]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{figures/convergence_of_modes_noise_r20_k8.png}
\end{subfigure}
\caption{Convergence of dominant modes, $r=5$, $r = 10$, $r = 20$. Bottom row includes noise} 
\label{fig:dominant_modes_conv}
\end{figure}


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\textcolor{blue}{merge with conclusions?}

\subsection{HODMD vs. MZMD}

\textcolor{blue}{move this to discussion section}
At this point, it is helpful to highlight the key differences between MZMD and HODMD, despite both methods increasing the spectral complexity relative to DMD. These distinctions arise both in the theoretical foundations and the algorithms employed. The HODMD assumption of the presence of higher-order Koopman is solely developed in the context of providing a modal decomposition technique so that the spectral complexity M can be greater than the spatial complexity N. With MZMD, this is no longer an assumption but a consequence of approaching a closure for DMD with the MZ formalism. MZMD provides a model of the states-space dynamics that can be derived within the MZ formalism which approximates a closure for DMD. Functionally, HODMD employs Taken’s delay embedding and a one-shot optimization to approximate the block companion matrix, along with an additional SVD truncation of the Hankel matrix of delay embeddings (which is not done is MZMD). This additional SVD truncation can, in some cases, break the original model assumption as we demonstrate in the next section. HODMD also faces challenges when applied to high-dimensional systems due to the curse of dimensionality, which increases computational complexity exponentially, limiting the amount of data that can be effectively analyzed. %Extensions of HODMD have thus be developed using tensor decompositions to address these issues \citep{li_hodmd_tensor2023}.

In contrast, MZMD approximates the modes and eigenvalues of the discrete-time GLE of state measurements (equation \eqref{eq_mz}) by leveraging the Mori-Zwanzig (MZ) formalism to construct an approximate closure model for DMD. This approach accounts for the interaction between unresolved variables and observables through the MZ memory kernels. Memory terms will almost always be non-trivial when applying MZMD to high dimensional nonlinear dynamical systems. Importantly, in MZMD, the first term remains equivalent to the DMD solution, even when memory effects are considered, and each term $\bm \Omega_i^{(g)}$ is learned separately, adhering to the MZ framework. This enforces the companion structure by construction, ensuring that the inclusion of MZ memory terms is directly additive to DMD and does not alter the results of the Markovian term ($\bm K$) derived from DMD, although the modes of MZMD and DMD are different when memory is included. %Moreover, algorithm \ref{alg:mzmd} incrementally minimizes the residual term in DMD.


A key difference, is that MZMD has additional interpretability provided by the memory terms, which explicitly account for how unresolved variables interact with resolved ones. Additionally, HODMD does not guarantee that the companion structure is preserved, whereas MZMD enforces this structure by construction. MZMD identifies individual memory terms that satisfy the MZ framework, particularly the GLE and the GFD. As we demonstrate in the next section, MZMD also offers a more efficient algorithm and can be more accurate for future state prediction. Additionally, while HODMD's algorithm \ref{alg:hodmd} relies on Takens' time-delay embeddings, MZMD does not. Thus, MZMD stands apart in both its theoretical foundation and algorithmic approach. Although, we demonstrate in the next section that time-delays and MZ memory are not mutually exclusive, and combining both can be advantageous. It is interesting to consider whether or not there exists a projection operator within the MZ framework, that bridges the gap, and establishes a theoretical connection between time-delay embeddings with MZ memory. However, a necessary condition that must be satisfied is the GFD, and within the current framework this currently requires an iterative approach for learning the MZ operators, as opposed to the joint optimization of time-delay embeddings.

\textcolor{blue}{move this last paragraph to discussion or results?}
If the second SVD that is performed on the Hankel matrix is truncated, then $\tilde{\bm R} $ may no longer satisfy the companion structure (numerical evidence of this shown in section \ref{sec:2d_cylinder}). This can happen, for example, when the number of time snapshots for fitting is less than $d*r_1$. In this case the maximum $r_2$ can be is $r_2 = T \leq d*r_1$ which forces $\hat{\bm G}$ to be a truncated SVD approximation. In this case, the HODMD algorithm could produce a coupled representation of past history which does not satisfy their original higher order Koopman assumption \eqref{eq:hodmd_assumption}, and provides a model that breaks causality. This is shown in more detail with numerical evidence in section \ref{sec:2d_cylinder}.This issue is not found in MZMD, and we discuss the theoretical and algorithmic differences in the next two sections.  






==> sections/mz_koopman.tex <==
\section{Koopman MZ}


As derived in \citep{lin2021datadriven_full}, the Mori--Zwanzig framework can be derived using the Koopman representation of the dynamics. Given a time $t\ge 0$, we would like to know how the resolved variables evolve in time $g_i(t; \bm x_0)$. Assuming the Koopman operator has a point spectra, the observables $g_i$ can be expressed as a linear combination of the countably infinite Koopman eigenfunctions (described in Sec.\ref{sec:koopman_background}) \cite{rowley2009SpectralAnalysisNonlinear,williams_2015_edmd}:
\begin{equation}
    g_i = \sum_{j=1}^\infty v_{i,j} \phi_j, \, i=1\ldots M. \label{eq:KoopmanEigDecomposition}
\end{equation}
As opposed to the equation \ref{eq:KoopmanEigDecomposition} which decompose a function into Koopman eigenfunctions, Mori--Zwanzig formalism utilizes the inner product in the Hilbert space to decompose the space into the subspace linearly spanned by the set of observables, $\Hilg:=\text{Span}(\MM)$, and an orthogonal subspace $\Hilgbar=\l\{\bar{g} \in \mathcal{F}: \l\langle \bar{g} , g_i\r\rangle=0, g_i \in \MM \r\}$. One proceeds with constructing a complete set of basis functions in $\Hil$, with a natural choice of using $\MM$ as the set of basis functions in $\Hilg$. One can then use the Gram-Schimidt process to construct the basis functions in the orthogonal space from the Koopman eigenfunctions, $\l\{\phi_i\r\}_{i=1}^{\infty}$. We denote this infinite set of basis functions by $\MMbar:=\l\{\bar{g}_i\r\}_{i=1}^\infty$. 
% Similar to Eq.~\eqref{eq:KoopmanEigDecomposition}, we can decompose $\bar{g}_i$'s in terms of the eigenfunctions: $\bar{g}_i = \sum_{j=1}^\infty \bar{v}_{i,j} \phi_j, \, i\in \mathbb{N}.$
% By construction, $\l\langle g_i, \bar{g}_j \r\rangle = 0$, $i \in \l\{1, \ldots, M\r\}$, $j \in \mathbb{N}$. Note that we did not require orthogonality between the basis functions in the same subspace, that is, $\l\langle g_i, g_j \r\rangle$ and $\l\langle \bar{g}_i, \bar{g}_j \r\rangle$ are not required to be $0$ if $i\ne j$. However, we assume linear independence between any of the pairs of the basis functions, and the combined set $\MM \cup \MMbar$ forms a complete set of basis functions in $\Hil$. 
It can be shown that any Koopman eigenfunction $\phi_i$ can be expressed in terms of these new basis functions
\begin{equation}
    \phi_i = \sum_{j=1}^M \omega_{i,j} g_j + \sum_{j=1}^\infty \bar{\omega}_{i,j} \bar{g}_j. 
\end{equation}
Applying the Koopman operator $\mathcal{K}_t$ to the above equation, we obtain the relationship $\forall t\ge 0$, $\phi_i(t) = \sum_{j=1}^M \omega_{i,j} g_j(t) + \sum_{j=1}^\infty \bar{\omega}_{i,j} \bar{g}_j (t)$. Expressing the evolution of the basis functions $g_i$, $i=1\ldots M$, the full dynamics can be described as 
% \begin{align}
%     \frac{d}{d t} g_i(t) = {}&\lim_{s\downarrow 0} \frac{\mathcal{K}_s g_i(t) - g_i(t) }{s} = \sum_{j=1}^\infty v_{i,j} \lambda_j e^{\lambda_j t} \phi_j = \sum_{i=0}^\infty v_{i,j} \lambda_j \phi_j(t)  \label{eq:giEvol} \\
%     ={}& \sum_{\ell=1}^M \l(\sum_{j=1}^\infty  v_{i,j} \lambda_j \omega_{j,\ell} \r) g_\ell(t) + \sum_{\ell=1}^\infty \l(\sum_{j=1}^\infty v_{i,j} \lambda_j \bar{\omega}_{j,\ell}\r) \bar{g}_\ell(t), \nonumber  
% \end{align}
% and similarly for $\bar{g}_i$, $i\in \mathbb{N}$:
% \begin{align}
%     \frac{d}{d t} \bar{g}_i(t) = \sum_{\ell=1}^M \l(\sum_{j=1}^\infty  \bar{v}_{i,j} \lambda_j \omega_{j,\ell} \r) g_\ell(t) + \sum_{\ell=1}^\infty \l(\sum_{j=1}^\infty \bar{v}_{i,j} \lambda_j \bar{\omega}_{j,\ell}\r) \bar{g}_\ell(t).  \label{eq:giBarEvol}
% \end{align}
% We have established that at any time, the evolution of $g_i(t)$ and $\bar{g}_i(t)$ are linear functions of themselves, which is the major consequence of the Koopman representation. We now adopt a terse vector notation $\bfvg_\MM\l(t\r)=\l[g_1(t),\ldots g_M(t) \r]^T$ and $\bfvg_\MMbar\l(t\r)=\l[\bar{g}_1(t), \bar{g}_2(t) \ldots \r]^T$ and concisely express the full dynamics as:
\begin{equation} 
\frac{d}{d t} \begin{bmatrix}
\bfvg_\MM(t) \\
\bfvg_\MMbar(t) 
\end{bmatrix}
=\bfvL\cdot \begin{bmatrix}
\bfvg_\MM(t) \\
\bfvg_\MMbar(t) 
\end{bmatrix}
:=
 \begin{bmatrix}
\bfvL_{\MM\MM} &  \bfvL_{\MM\MMbar} \\
\bfvL_{\MMbar\MM} & \bfvL_{\MMbar\MMbar}\
\end{bmatrix}
\cdot
 \begin{bmatrix}
\bfvg_\MM(t) \\
\bfvg_\MMbar(t) 
\end{bmatrix}, \label{eq:fullKoopman}
\end{equation}
where $\bfvg_\MM\l(t\r)=\l[g_1(t),\ldots g_M(t) \r]^T$ and $\bfvg_\MMbar\l(t\r)=\l[\bar{g}_1(t), \bar{g}_2(t) \ldots \r]^T$. Here, the matrices $\bfvL_{i,j}$, $i,j \in \l\{\MM,\MMbar\r\}$, quantifies the effect from set $j$ to set $i$ in the linear evolution. %While these matrices can be found explicitly from Eqs.~\eqref{eq:giEvol} and \eqref{eq:giBarEvol} should one know the Koopman eigenfunctions, we derive them just for the purpose of establishing the linear evolutionary equation \eqref{eq:fullKoopman}. 
Although $g_i(0)=g_i \in \Hilg$ and $\bar{g}_i(0)=\bar{g}_i \in \Hilgbar$,  for $t>0$, $g_i(t)$ and $\bar{g}_i(t)$ are not necessarily in $\Hilg$ and $\Hilgbar$ respectively, if the interactions between the spaces, $\bfvL_{\MM\MMbar}$ and $\bfvL_{\MMbar\MM}$, are not zero. In other words, in general, both $g_i(t)$ and $\bar{g}_i(t)$ have nonzero components of the basis functions in $\Hilg$ and $\Hilgbar$. Nevertheless, the above linear equation \eqref{eq:fullKoopman} always holds.  

To obtain a closed-form evolution for our observables of interest in $\MM$, we first solve for the observables in set $\MMbar$  implicitly. Treating $\bfvL_{\MMbar\MM} \bfvg_\MM$ as an inhomogeneous driving term of the linear system, we solve the linear evolutionary equation for $\bfvg_\MMbar$:
\begin{align}
\bfvg_\MMbar(t) ={}&  \int_0^t e^{\l(t-s\r) \bfvL_{\MMbar\MMbar}} \cdot \bfvL_{\MMbar\MM}\cdot\bfvg_\MM(s) d s+e^{t \bfvL_{\MMbar\MMbar}} \cdot \bfvg_\MMbar(0). \label{eq:underResolvedDynamics}
\end{align}
The implicit solution of $\bfvg_\MMbar$ is in turn used to express closed evolutionary equations for the observables in the set $\MM$. 
\begin{align}
\frac{d}{d t} \bfvg_\MM(t) ={}& \bfvL_{\MM\MM} \bfvg_\MM\l(t\r) +\bfvL_{\MM\MMbar}\int_0^t e^{\l(t-s\r) \bfvL_{\MMbar\MMbar}} \cdot \bfvL_{\MMbar\MM}\cdot\bfvg_\MM(s) d s \label{eq:pGLE}  \\
{}& +\bfvL_{\MM\MMbar} e^{t \bfvL_{\MMbar\MMbar}} \cdot \bfvg_\MMbar(0).  \nonumber 
\end{align}
Equation \eqref{eq:pGLE} is almost closed in our chosen set of variables except for the last term. The first term is the instantaneous configuration of the set of observables applied to the physical-space configuration at time $t$ and the second is a delayed impact of the set of observables applied to the physical-space variables at an earlier time $s<t$. Both these terms depend only on the resolved observables $\bfvg_\MM$ at time $t$. However, the third term is induced by the initial setting of the under-resolved observables, $\bfvg_\MMbar(0)$, which cannot be generally resolved. Equation \eqref{eq:pGLE} is exact if one knows both $\bfvg_\MMbar(0)$ and $\bfvg_\MMbar(0)$, in which case, the system is fully resolved. Unfortunately, we do not have direct access to $\bfvg_\MMbar(0)$ as they are under-resolved observables, and one has to postulate their configurations in practice. 

This simple analysis illustrates the essential intuition of the Mori--Zwanzig formalism. Because we only resolve a set of observables $\bfvg_\MM(t)$ of the full dynamics, the impact from other observables $\bfvg_\MMbar(t)$ in Eq.~\eqref{eq:fullKoopman} cannot be directly accessed. Instead, we indirectly estimate the effect $\bfvL_{\MM\MMbar}\cdot \bfvg\l(t\r)$ from Eq.~\eqref{eq:underResolvedDynamics}, which contains two parts: the impact of resolved observables $\bfvg_\MM(s)$ at an earlier time $s$, and the initial conditions of the orthogonal observables $\bfvg_\MMbar$. The former characterizes the ``echo'' of the set of our interested observables to itself: at an earlier time $s$, these observables made an impact to the under-resolved observables $\bfvg_\MMbar$ (via $\bfvL_{\MMbar\MM}$), and such an impact propagates among the under-resolved observables $\bfvg_\MMbar$ for $t-s$ time via $e^{(t-s) \bfvL_{\MMbar \MMbar}}$ before coming back to affect the resolved observables at time $t$ via $L_{\MM\MMbar}$. The second part is a generic impact from the initial configuration of the orthogonal set of observables, $\bfvg_{\MMbar}(0)$, which has propagated in the under-resolved observables until the current time $t$ and affects the resolved observables. In the end, Eq.~\eqref{eq:pGLE} tells us that the accurate evolutionary equations of $\bfvg_\MM(t)$ always depend on (1) their instantaneous configuration, (2) their past history, and (3) an external ``driving force'' which depends on the initial configurations in the orthogonal space. 

We make a remark that the second and the third term are zero if the dynamics is closed in $\MM$, that is, $\bfvL_{\MM \MMbar}=0$ which corresponds to the scenario when we have a complete set of observables to describe the full dynamics. For example, this would be the $g_e:=\exp(-1/x)$ for the dynamics $\dot{x}=-x^2$. The memory and the external driven force exist only because we have an incomplete observable set in $\Hil$. 

We now drop the subscript $\MM$ in $\bfvg_\MM$, as we only care about the dynamics of the resolved observables. By defining an $M\times M$ matrix $\bfvM:=\bfvL_{\MM\MM}$, an $M\times M$ matrix parametrized by $\bfvK\l(s\r) :=- \bfvL_{\MM\MMbar} e^{s \bfvL_{\MMbar\MMbar}} \cdot \bfvL_{\MMbar\MM}$ parametrized by $s\in \mathbb{R}^+$, and an $M\times 1$ matrix $\bfvF(t):=\bfvL_{\MM\MMbar} e^{t \bfvL_{\MMbar\MMbar}} \cdot \bfvg_\MMbar(0)$, we arrive at the GLE
\begin{equation}
\frac{d}{d t} \bfvg\l(t\r) = \bfvM \cdot \bfvg\l(t\r) - \int_{0}^t \bfvK\l(t-s\r)\cdot \bfvg\l(s\r)d s + \bfvF\l(t\r).\label{eq:GLE}
\end{equation}
In the rest of the paper, we refer to $\bfvM$ as the \emph{Markov transition matrix}, $\bfvK(s)$ as the \emph{memory kernel}, and $\bfvF(t)$ as the \emph{orthogonal dynamics}. Although $\bfvF(t)$ is fully deterministic in Mori--Zwanzig formalism for deterministic systems, it is often referred to as the \emph{noise} because its resemblance of a Langevin noise in a Langevin equation. Note that the operators $\bfvM$ quantify the interactions within the group of the relevant observables $\l\{g_i\r\}_{i=1}^M$ (that is, $\bfvL_{\MM \MM}$). In contrast, the memory kernel combines the effects of the rest of the interactions ($\bfvL_{\MM \MMbar}$, $\bfvL_{\MMbar \MM}$, and $\bfvL_{\MMbar \MMbar}$)

Finally, we remark that despite their different terminologies, Eq.~\eqref{eq:GLE} and the operator algebraic formulation Eq.~\eqref{eq:opGLE} are equivalent. When $g_i(\bfv{x})=x_i$, given an initial condition $\bfvPhi_0$, $g_i\circ \bfvPhi_0$ in Eq.~\eqref{eq:GLE} \emph{is} $\phi_i \l(t, \bfvPhi_0\r)$ in Eq.~\eqref{eq:opGLE}. 



==> sections/mz_mori_projector.tex <==
\subsection{Mori's Projection}
The difference between Mori and Zwanzig is their choice of the projection operator. With Mori's construction \cite{mori1965transport}, one relies on an inner product defined as 
\begin{equation}
    \left\langle f, g \right\rangle = \int_{\mathbb{R}^N} f\left(\bm {x}\right) g\left(\bm {x}\right) \rho\left(\bm {x}\right) d^N \bm {x}, \quad f, g\in L^2\left(\mu \right) \label{eq:MoriInner}
\end{equation}
to define a projection operator given a set of resolved observables $\hat{x}=\left\{x_i \right\}_{i=1}^M$:
\begin{equation}
    \left[\mathcal{P} f\right] \left(\hat{x} \right) := \sum_{i,j=1}^M \left\langle f, x_i \right\rangle \left[\bm C^{-1}_0\right]_{i,j} x_j.
\end{equation}
where $\bm C^{-1}(0)$ is the inverse of an $M\times M$ matrix $\bm {C}_0$ whose $(i,j)$ entry is $\left\langle x_i, x_j \right\rangle$. Note that $\mathcal{P} f $ is a linear function of the resolved observables, $x_j$, $j=1\ldots M$, and thus Mori's projector is often referred to as a linear projection. In contrast, with the same set of observables, Zwanzig \cite{zwanzig1973nonlinear} does not rely on the inner product but relies on the direct marginalization of the under-resolved observables \citep{lin2021datadriven_full}. 
After applying Mori's projection operator to $M$, $F$, and $K$, one obtains a linear GLE \cite{zwanzig_nonequilibrium_2001}: 
\begin{equation}
    \frac{d}{d t} \hat{x}_i(t, \bm x_0)
    = \sum_{j=1}^M \left[\bm M\right]_{i,j} \hat{x}_j\left(t, \bm x_0\right) - \int_0^t \left[\bm K(t-s)\right]_{i,j} \hat{x}_j\left(t, \bm x_0\right) d s + F_i(t, \bm x_0).  \label{eq:opGLE}
\end{equation} 
where $\bm M$ is an $M\times M$ constant matrix, as well as $\bm K(t)$, $t\ge 0$. In this manuscript, we will be applying Mori's projection.

Both the Koopman \cite{koopman_hamiltonian_1931, koopman_dynamical_1932} and Mori--Zwanzig formulations operate in a Hilbert space, whose inner product is commonly defined as the inner product of two functions as the expected value of the product of the two with respect to a chosen measure $d \mu$, Eq.~\eqref{eq:MoriInner}. Despite of the freedom to choose this measure, $d \mu$ is conventionally set as a natural measure that is specific to the dynamics. For example, it is natural to adopt the canonical equilibrium distribution (Gibbs' measure) for equilibrium Hamiltonian systems \cite{mori1965transport}. For non-equilibrium systems, we can adopt the stationary measure as $d \mu$ \cite{evans2007statistical}, as shown below. For stochastic and transient systems, it is natural to choose the induced time-dependent distribution \cite{wu2020VariationalApproachLearning}.

With a defined inner product, Mori used an operator $\mathcal{P}$ that projects any function (of the initial condition $\bfvPhi_0$) $f \in \Hil$, onto the subspace $\Hilg:=\text{span}\l(\MM\r)=\text{span}\l(\l\{g_i\r\}_{i=1}^M\r)$. As such, the projected image can be expressed by $\mathcal{P} f := \sum_{i=1}^M \alpha_i g_i$ with coefficients $\alpha_i$. Now, we decompose the function $f$ by $ f= \mathcal{P} f + f_\perp$ where $f_\perp \in \Hilgbar$. Because $\l\langle f_\perp, g_j \r\rangle=0$, $j=1\ldots M$, the inner product $\l\langle f, g_j \r\rangle$ is:
\begin{equation}
\l\langle f, g_j \r\rangle = \l\langle \mathcal{P} f, g_j \r\rangle  = \sum_{i=1}^M \alpha_i \l\langle g_i, g_j \r\rangle.  \label{eq:innerProduct}
\end{equation}
In vector notation, $\bfvg:=\l[g_1 \ldots g_M\r]^T$ and $\bfv{\alpha}:=\l[\alpha_1 \ldots \alpha_M\r]$, the above equation can be expressed concisely by $\l\langle f, \bfvg^T \r\rangle= \bfv{\alpha} \cdot \l\langle \bfvg, \bfvg^T \r\rangle$. Because the basis functions $g_i$'s are linearly independent, $\l\langle \bfvg , \bfvg^T \r\rangle$ is a full-rank and invertible matrix. Then, $\bfv{\alpha}=\l\langle f, \bfvg^T \r\rangle \cdot  \l\langle \bfvg , \bfvg^T \r\rangle^{-1}$, and we obtain the final expression for the projection operator
\begin{equation}
\mathcal{P} f = \l\langle f, \bfvg^T \r\rangle \cdot  \l\langle \bfvg , \bfvg^T \r\rangle^{-1} \cdot \bfvg.
\end{equation}
Note that if and only if the pre-selected set of functions $\l\{g_i\r\}_{i=1}^M$ are orthonormal with respect to the defined inner product, $ \l\langle \bfvg , \bfvg^T \r\rangle^{-1} $ is an identity matrix and the expression can be simplified by $\mathcal{P} f=\l\langle f, \bfvg^T \r\rangle   \cdot \bfvg$. Finally, we emphasize that the projection operator crucially depends on the choice of the defined inner product. In the rest of this article, we consider an inner product defined by averaging the observables over a long trajectory of the dynamical system:
\begin{equation}
\l\langle f , g\r\rangle := \lim_{T\rightarrow \infty}\frac{1}{T} \int_0^T \l(f\circ \bfvPhi(s) \r) \l( g\circ \bfvPhi(s)\r) d s, \label{eq:ctsInnerProduct}
\end{equation}
where $\bfvPhi\l(t\r)$ is the solution of Eq.~\eqref{eq:phiEvo} from any initial condition, assuming the choice of the initial condition does not change the long-time statistics. 

